Normalizing Compositional Structures Across Graphbanks

The emergence of a variety of graph-based meaning representations (MRs) has sparked an important conversation about how to adequately represent semantic structure. These MRs exhibit structural differences that reflect different theoretical and design considerations, presenting challenges to uniform linguistic analysis and cross-framework semantic parsing. Here, we ask the question of which design differences between MRs are meaningful and semantically-rooted, and which are superficial. We present a methodology for normalizing discrepancies between MRs at the compositional level (Lindemann et al., 2019), finding that we can normalize the majority of divergent phenomena using linguistically-grounded rules. Our work significantly increases the match in compositional structure between MRs and improves multi-task learning (MTL) in a low-resource setting, demonstrating the usefulness of careful MR design analysis and comparison.

==> notes.tex <==
\textbf{Notes}

\begin{enumerate}
    \item \textbf{Background/Technical contribution:} we have good reason to \todo{old: modify the AM algebra} unify the underlying representations of distinct graphbanks to increase accuracy and generalizability of our semantic parser, but this is not as easy as it seems.
    \item \textbf{Top 3-5 tricky linguistic phenomena} with detailed examples of how we remedy (e.g. negation from Alexander's DMR talk).
    \item \textbf{Quantify:} what discrepancies can we find structurally and compositionally? Cite data from shared drive. This is where we discuss structural patterns vs. linguistic patterns.
    \item \textbf{Unify.} Based on previous step, linguistic intuitions, etc. 
    \item \textbf{Reevaluate} parser with updated heuristics, with MTL if time permits. \todo{latest by 4 April}
    \item \textbf{GOAL:} MTL across banks taking small sample of one. This would hopefully simulate a low-resource graphbank. Will also hopefully support the compositional nature of our parser that is linguistically rooted, to capture important generalizations. Though more data will always help, the unification of the dependency trees allows MTL to help our performance more than e.g. Dozat and Manning. \todo{latest by 27 March}
    \item \textbf{Other:} joint decoding?
    \item \textbf{Conclude:} graph banks now have consistent AM trees, hopefully this increases F-score.
    \item Future work = multitask learning.  
    \end{enumerate}
\textbf{Page breakdown:} 
        \begin{itemize}
            \item Introduction: 1 page
            \item Background/Related Work: 1 page
            \item Description of patterns (3 pages total): 1.5 pages / linguistic phenomena; 1.5 pages / structural patterns (integrated). TO DO: what are the connections here? Create document. Consider how interactions occur; perhaps we need to adjust in a specific order.
            \begin{itemize}
                \item Determiners \ld{done - write description}
                \item Negation  \ml{Matthias once able to}\ld{\textbf{update:}look at different types of negation, diff sources}
                \item Prepositions \textbf{by March 18}
                \item Coordination (2+ and 3+) \textbf{by March 18}
                \item Copula \pw{Pia for \textbf{March 11}}
                \item Punctuation \pw{Pia for \textbf{March 11}}
                \item Modals and auxiliaries \jg{Jonas} \textbf{by March 11}
                \item General headedness of NPs and MWEs (if time). Also applies to copula, coordination, negation. Prepositions? \pw{\ld{Update}: Continue discussion} 
                \item \textbf{General for all:} think about how to remedy general issues
            \end{itemize}
            \item Quantification and unification: 1 page (more focused on table)
            \item Reevaluation: .5 page (table
            \item MTL: 1 page 
            \item Conclusion: .5 page
        \end{itemize}



           
           

\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Signature & Frequency & POS tags      & Linguistic construction                                                                                          \\ \midrule
777       & 9918 \ld{correct?}      & NN, NNS, NNP  & Common nouns \textit{(same treatment across MRs)                                              }                            \\
660       & 60454     & DT, RBR, RBS  & Determiners \textit{(ignored by PSD)  }                                                                                    \\
220       & 51301     & IN, TO, VBG   & Prepositions \textit{(ignored by PSD)  }                                                                                     \\
020       & 27840     & IN, POS, TO   & Prepositions \textit{(some ignored by DM)  }                                                                                 \\
111       & 22543     & VBD, VB, VBZ  & Transitive verbs \textit{(same treatment across MRs)}                        \\
012       & 11040     & CC, ",", IN   & Coordination \textit{(PSD converted to PAS)} \\
675       & 7376      & NNP, CD, NN   & Named entities\jg{not sure they are NEs}                                                                                                   \\
120       & 6974      & IN, TO, WRB   & Prepositions \textit{(subordinating conjunctions)                                        }                               \\
022       & 5656      & ",", CC, :    & Coordination                                                                                                     \\
540       & 4363      & MD, VBD, VBP  & Modal verbs                                                                                                      \\
031       & 3467      & VBZ, VBD, VBP & Copula  \pw{add observation}                                                                                                        \\ \bottomrule
\end{tabular}
\caption{Selection of most frequent patterns and their makeup found in data across MRs. Signatures represent graph type by MR, in order left to right: DM, PAS, PSD. \ld{Explain graph type by number.}}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
                        & \multicolumn{1}{l}{Phenomenon}    & Example \ld{(give 2-way example)}
                        & Frequency 
                        \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Type 0\\ (handled by AM 2019)\end{tabular}}             & \begin{tabular}[c]{@{}l@{}}\textbf{Edge Labels}\\ (Partial)\end{tabular}       &                              &           \\                                 & \begin{tabular}[c]{@{}l@{}}\textbf{Adjectives}\\ (Edge direction)\end{tabular} &                              &           \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Type 1\\ (simple fix)\end{tabular}}    & \textbf{Determiners}                         &       \includegraphics[scale=.5]{determiners.png}         & 60k       \\
                                                                                                   & \textbf{Punctuation}        &     \ld{PAS treats with ModPunct; others ignore}                         & 58k       \\ \midrule
\multirow{2}{*}{Type 2}                                                                            & \begin{tabular}[c]{@{}l@{}}\textbf{Auxiliaries}\\ Temporal\end{tabular}        &                              & 18k       \\
                                                                                                   & Modal                                                                 &                              & 4k        \\ \midrule
\multirow{5}{*}{Type 3}                                                                            & \begin{tabular}[c]{@{}l@{}}\textbf{Coordination}\\ 2 conjuncts\end{tabular}    &                              & 27k       \\
                                                                                                   & 3+ conjuncts                                                          &                              & 3k        \\
    &\begin{tabular}[c]{@{}l@{}}\textbf{Prepositions}\\ General\end{tabular}        &                              & 51k       \\
                                                                                                   & Possessives                                                           &                              & 28k       \\
                                                                                                   & Other                                                                 &                              & 7k?       \\ \midrule
\multirow{2}{*}{Type 4}                                                                            & \textbf{Negation}                                                              &                              & 4k?       \\
                &\begin{tabular}[c]{@{}l@{}}\textbf{Copula}\\ Adjectival\end{tabular}         &                              & 3.4k      \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Type 5\\ (not considered\\ in this paper)\end{tabular}} & Appositions                                                           &                              &           \\
                                                                                                   & MWEs                                                                  &                              & 40K +     \\
                                                                                                   & Relative Pronouns                                                     &                              &           \\
                                                                                                   & Other...                                                              &                              &           \\ \bottomrule
\end{tabular}
\caption{Frequency of mismatched patterns across DM, PAS, and PSD graphbanks by linguistic type. Examples show mismatches as they are construed by the AM algebra in AM dependency trees.}\label{tab:patternfreq}
\end{table} 

==> pics/cutecatsanddogs.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{.22\linewidth}
		\centering
		\begin{dependency}[sdpgraph]
			\begin{deptext}%[column sep=.5em]
				Cute \& cats \& and \& dogs \\
			\end{deptext}
			\deproot[edge unit distance=1.3ex]{2}{ROOT}
			\depedge[edge unit distance=1ex]{1}{2}{ARG1}  % cute cats
			\depedge[edge unit distance=1ex]{2}{4}{\_and\_c} % (and) cats dogs
		\end{dependency}
		\caption{DM, ambiguous scope}\label{fig:ambigDM}
	\end{subfigure}
	\begin{subfigure}[b]{.38\linewidth}
		\centering
		\begin{dependency}[sdpgraph]
			\begin{deptext}[column sep=2em]
				Cute \& cats \& and \& dogs \\
			\end{deptext}
			\deproot[edge unit distance=1.5ex]{3}{ROOT}
			\depedge[edge unit distance=1ex]{1}{2}{adj\_ARG1}  % cute cats (narrow scope)
			\depedge[edge unit distance=2ex]{3}{2}{coord\_ARG1}  % cats and
			\depedge[edge unit distance=2ex]{3}{4}{coord\_ARG2}  % and dogs
		\end{dependency}
		\caption{PAS, narrow scope}\label{fig:ambigPASnarrow}
	\end{subfigure}
	\begin{subfigure}[b]{.38\linewidth}
		\centering
		\begin{dependency}[sdpgraph]
			\begin{deptext}[column sep=2em]
				Cute \& cats \& and \& dogs \\
			\end{deptext}
			\deproot[edge unit distance=1.5ex]{3}{ROOT}
			\depedge[edge unit distance=1.5ex]{1}{3}{adj\_ARG1}  % cute and (wide scope)
			\depedge[edge unit distance=1ex]{3}{2}{coord\_ARG1}  % cats and
			\depedge[edge unit distance=2ex]{3}{4}{coord\_ARG2}  % and dogs
		\end{dependency}
		\caption{PAS, wide scope}\label{fig:ambigPASwide}
	\end{subfigure}
	\caption{Coordination and its representation of scope in DM and PAS.
	%Cute cats and dogs, DM and PAS graphs
	}
	\label{fig:ambig}
\end{figure}

==> pics/figuremacros.tex <==

\usepackage[T1]{fontenc}     %% font encoding  have umlaut ä as one symbol, not a"
\usepackage[utf8]{inputenc}  %% input encoding  write umlaut ä as ä instead of \"a
\usepackage[english]{babel}  %% important for hypenation among others
\usepackage{graphicx}  %% for inserting graphics

\usepackage{tikz-dependency}
\depstyle{amdep}{label style={text=black, fill=black!10}, edge style={thick}, edge slant=1pt}% theme=night,  theme=default
\depstyle{sdpgraph}{text only label, label style={font=\small\slshape, above}, edge style={>=latex,solid,gray}, edge slant=5pt}
%\depstyle{amdep}{theme=default} % old
%\depstyle{sdpgraph}{text only label, label style={font=\small, above}} % old
\usepackage{amsmath}  %% math packages
\usepackage{amsfonts}
\usepackage{amssymb}

\newcommand{\s}[1]{$_\textsc{#1}$}

\usepackage{forest}
\usepackage{float}
%subfigures
\usepackage{caption}
\usepackage{subcaption}

\usepackage{xspace}

% AM algebra things:
\newcommand{\sources}{\ensuremath{\mathcal{S}}}
\newcommand{\tp}[1]{\ensuremath{\tau(#1)}}   % type variable
\newcommand{\type}[1]{\ensuremath{[#1]}}

\newcommand{\rename}[1]{\text{ren}\ensuremath{_{#1}}}    %\rename{\src{a}\mapsto \src{b}}
\newcommand{\forget}[1]{\ensuremath{f_{\scriptsize#1}}}                          %\forget{\src{a}} 
\newcommand{\mg}{\ensuremath{~||~}\xspace}

\newcommand{\app}[1]{\text{\textsc{App}}\ensuremath{_{#1}}}  %\app{arg}
\newcommand{\modify}[1]{\text{\textsc{mod}}\ensuremath{_{#1}}\xspace}
\newcommand{\lignore}{\text{\textsc{ignore}}}

% source

\newcommand{\src}[1]{\text{\textsc{#1}}\xspace}                                  % source name 
\newcommand{\obj}[1][]{\text{\src{o}}\ensuremath{_{#1}}}               % object sources. \obj or \obj[i]
\newcommand{\subj}{\text{\src{s}}}													% subject source, just \subj
\newcommand{\op}[1][i]{\text{\src{op}}\ensuremath{_{#1}}}			% op sources \op[i]
\newcommand{\rt}{\src{rt}}


\newcommand{\G}[1]{\ensuremath{G_{\text{#1}}}} % naming graphs
\newcommand{\elem}{\ensuremath{T}}  % set of predicted elementary graphs
\newcommand{\ops}{\ensuremath{O}}  % set of predicted operations

\newcommand{\of}[1]{\left(#1\right)}

\newcommand{\todo}[1]{\textcolor{red}{\textbf{(#1)}}}%{}%
 

%% graph and tree drawing
\usepackage{tikz}
\usepackage{tikz-qtree}



==> pics/tex/catnotlazy_amalgebra.tex <==
% \documentclass{article}
% \input ./figuremacros.tex
% \begin{document}


\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\linewidth} % {0.6\linewidth} 
		\centering
		\includegraphics[scale=1.1]{../pdf/PAS_copula}\hspace{-5pt}
		\includegraphics[scale=0.8]{../pdf/PAS_lazyS}\hspace{-10pt}
		\includegraphics[scale=0.4]{../pdf/cat}
		\includegraphics[scale=0.8]{../pdf/PAS_the}\hspace{-10pt}
		\includegraphics[scale=0.8]{../pdf/PAS_notOld}
		\caption{Constants \G{be}, \G{lazy}, \G{cat}, \G{the}, and \G{not}}\label{fig:am:consts}
	\end{subfigure}
	\begin{subfigure}[b]{.25\linewidth}
		\centering
		\includegraphics[scale=0.35]{../pdf/belazyPAS}
		\caption{$\app{\src{O}}\of{\G{be},\G{lazy}}$}\label{fig:am:beLazy}
	\end{subfigure}
	\begin{subfigure}[b]{.25\linewidth}
		\centering
		\includegraphics[scale=0.35]{../pdf/thecatPAS}
		\caption{$\modify{\src{det}}\of{\G{cat},\G{the}}$}\label{fig:am:theCat}
	\end{subfigure}
	
	\begin{subfigure}[b]{0.2\linewidth} %0.3 {0.3\linewidth} 
		\centering
		\includegraphics[scale=0.4]{../pdf/fullgraphPAScatnotlazy}
		\caption{PAS graph}\label{fig:am:graph}
	\end{subfigure}
	\begin{subfigure}[b]{.35\linewidth} % {0.3\linewidth}
		\begin{center}
			\resizebox{.5\linewidth}{!}{
			\begin{forest}
				for tree={align=center, l=\baselineskip, l sep=5pt} % l: parent-child, s: sibling distance
				[{\modify{\src{mod}}}, for tree={fill=green!30}
					[{\app{\src{s}}}, for tree={fill=green!30}
						[{\app{\obj}}
							[{\G{be}},tier=word]
							[{\G{lazy}}, for tree={fill=red!30},tier=word]
						]
						[{\modify{\src{det}}}, for tree={fill=brown!10!yellow!60}
							[{\G{cat}},tier=word]
							[{\G{the}}, for tree={fill=blue!30},tier=word]
						]
					]
					[{\G{not}}, for tree={fill=orange!30},tier=word]
				]
			\end{forest}}
		\end{center}
		\caption{AM term}\label{fig:am:term}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\linewidth} % {0.5\linewidth}
		\begin{center}
			\resizebox{.7\linewidth}{!}{
			\begin{forest}
				for tree={draw,align=center, no edge, s sep=15pt}
				[parent, phantom
				[{\G{the}\\The}, name=the, fill=blue!30]
				[{\G{cat}\\cat}, name=cat, fill=brown!10!yellow!60]
				[{\G{be}\\is}, name=be, fill=green!30]
				[{\G{not}\\not}, name=not, fill=orange!30]
				[{\G{lazy}\\lazy}, name=lazy, fill=red!30]
				]
				\draw[->] (be) to[out=north, in=north, edge node={node[above, fill=green!30] {\modify{mod}}}] (not);
				\draw[->] (be) to[out=north, in=north, edge node={node[above, fill=green!30] {\app{\src{S}}}}] (cat);
				\draw[->] (be) to[out=north, in=north, edge node={node[above, fill=green!30] {\app{\obj}}}] (lazy); %60 out, 1110 in
				\draw[->] (cat) to[out=north, in=north, edge node={node[above, fill=brown!10!yellow!60] {\modify{\src{det}}}}] (the);%pos=0.65,
			\end{forest}}
		\end{center}
		\caption{AM dependency tree}\label{fig:am:deptree}
	\end{subfigure}
	\caption{PAS for \textit{the cat is not lazy} with its AM analysis. \todo{reformat to save space}. Simplified (\src{s} instead of \src{mod} source for adjective)}\label{fig:am}
\end{figure}

%\end{document}

==> unification_old.tex <==

\section{Updating the Heuristics}\label{sec:updating} 

\ak{This introduction does a good job of explaining how we are going to \emph{solve} the problem. It needs a clear statement of the problem itself to push off from.}

\jg{My rewrite of this lacks motivation, I think some of the text here could help it out.}

We update the heuristics of the AM algebra and parser with two sets of questions in mind: (i) Which graphbank design choices capture real linguistic information and should be maintained? Which choices can be replaced by another without losing important information? (ii) How do these design choices impact parsing? Can we make parsing more accurate by converting between representation styles during pre- and post-processing? \jg{With our parsing results being not too impressive, maybe we shouldn't put the spotlight on them here?}

These questions go hand in hand: as we investigate specific constructions of interest for their linguistic complexity, we find that these same constructions are reflected in patterns that emerge from statistically analyzing differences in parser output. Thus, we first quantify discrepancies between the AM dependency trees that we use as our intermediate parsing step; this allows us pinpoint patterns that impact our parsing accuracy separate from their strict linguistic import (section \ref{subsec:quantifying}). In approaching specific linguistic constructions, we confront challenges unique to the AM algebra and how it is able to decompose linguistic structure. We qualitatively investigate four key representational differences between the three MRs in question for specific complex linguistic constructions known to cause parsing difficulty, outlining how we remedy them (section \ref{subsec:lingstructures}). 

\subsection{Quantifying the phenomena}\label{subsec:quantifying}

\ak{I wonder if this can be explained better from examples. As it stands, the detection criteria fall out of the sky a bit. What are we actually trying to detect? What does that look like e.g.\ in the determiner examples above? Are the criteria at the level of teh graphs or of the AM deptrees? Does it matter, and why?}

%As part of our goal is to improve parsing accuracy, 
\ld{Change to reflect updated signature with AM dependency trees:}
We conduct a pattern analysis of our data to identify the frequency and nature of representational discrepancies between the MRs. To do this, we use three pieces of information for our detection criteria: (i) POS tags and lemmas that allow us to identify the tokens involved in the construction; (ii) the incoming edge label to the node, which allows us to distinguish whether the node is a head (with an incoming \textsc{App} edge), a modifier (with an incoming \textsc{Mod} edge), or ignored (with an incoming \textsc{ignore} edge); and (iii) the number of \textsc{App(ly)} children, which allows us to identify how many arguments a node has. This information is translated into numeric form: the manner in which a MR treats a certain phenomenon is represented by a number that corresponds to a graph pattern in the AM algebra. As each MR then has a number for a phenomenon, we get unique \textit{signatures} of graph patterns by linguistic construction and obtain the frequency of these pattern combinations. For example, the signature \textit{777} is observed for 99,189 cases with the most common POS tags being NN, NNS, and NNP. This signature tells us that all three MRs represent common nouns with a source graph that possesses no outgoing \textsc{App} edges. More signatures, their frequencies, and an explanation of graph type by number are explained in Table \ref{tab:patternfreq}. \pw{maybe mention complication through headedness or interaction of phenomena: maybe there are more e.g. copula, but we don't detect all in one pattern because of interactions with other phenomena?} \ak{We can only talk about 777 here if we explain at least for 7 what a ``graph pattern'' looks like.}


The statistical patterns we observe reflect known linguistic constructions in intriguing ways. For example, while the treatment of determiners conforms to the observation above that DM and PAS treat them in a unified manner (as AM \textsc{Modifiers}) and PSD ignores them, phenomena like prepositions and copula are more varied in how the MRs represent them. In other words, our statistical analysis allows us to capture refined distinctions that exist within canonical linguistic categories. Taking prepositions as an example, we see that, though PSD tends to ignore them, the differences in their representation between DM and PAS is more patterned than perhaps a manual analysis by type would uncover. 
\ld{Add bit about phenomena not included / Zipfian tail}



%\begin{itemize}
    
 %   \item Describe process of identifying patterns, comparing between graphbanks, adjusting the individual blobs to be least offensive \todo{Pia} and \todo{Lucia}
  %  \item Can we get sources from different graphbanks to be more consistent/similar? E.g. APPoo in PSD is an outlier that seems to cause many differences between PSD/DM and PSD/EDS \todo{some source names like oo in PSD are only present in one framework, therefore mismatch as least as big as summed frequency of these framework-specific sources}
   % \item \todo{other advantages of AMplus algebra? can we make the non-decomposablility problem for EDS smaller?}
   

%\end{itemize}

%\subsection{Challenges with the AM Algebra}\label{subsec:challengesam}





\subsection{Key Phenomena}\label{subsec:lingstructures} 

\ld{combined previous section here, so this part all needs to be better integrated}
Complementary to our observations from the statistical patterns in the data, we notice qualitative structural patterns shared across select representations for certain linguistic constructions. For example, whether one element is considered to be a modifier or the head of another element results in \textit{head-modifier} problems. Negation of a verb is such a problem: PSD and PAS treats negation as a verbal modifier, whereas in DM treats negation as the head of the verb. %discourse connectors? 


These structural patterns raise several challenges unique to the compositional nature of our parsing task. First, the question arises as to how to optimally label the sources of the individual as-graphs and assign supertags. The heuristics developed in \newcite{lindemann2019compositional} are framework-specific, which often leads to different supertag types for any given word. Although the unlabeled AM dependency trees across MRs are structurally equivalent, the labeled ones are not. This issue applies to phenomena such as MWEs and adverbial modification: for example, in the sentence \textit{The bear wandered slowly}, all three AM dependency trees possess a \textsc{Mod} edge pointing from \textit{wandered} to \textit{slowly}, but they differ slightly in their edge labels (DM as \textsc{Mod\textsubscript{s}}, PAS and PSD as \textsc{MOD\textsubscript{Mod}}) as well as in the as-graph for \textit{slowly}. Here, it is unclear whether there is a trade-off between simplifying our supertag lexicon in favor of more uniform AM dependency trees, or if perhaps we can achieve both simultaneously. \ld{Add visual? Others can add more precise thoughts here.} \ak{Supertags are not yet explained in the paper. I think as a reader, I really want to see now how you do it; I don't want to hear about limitations or design choices. I would get to the point quickly here, and then discuss limitations, alternatives, and interactions below. Keep it as simple here as you can.}

%Additionally, coordination and copula are both instances of \textit{linker} problems where one MR chooses to not represent the contribution of the \textit{linking element} (e.g. the coordinator or the copula verb), and instead directly connects the items; %\pw{in our current dependency tree and supertag lexicon the linker seems to be ignored, but actually in graph you can observe coordination, but not any copula related edge or node in DM}; 
%in contrast, another MR takes the linker to be the central element (root of the subgraph or head of the dependency subtree) connecting the items. 

%\ml{Matthias:}A trade-off between simpler supertag lexicon and more uniform AM dep trees? new measure that our new results are actually better (good supertags \textbf{and} dep trees)?

Additional challenges arise when we attempt to unify more structurally rooted discrepancies such as distinct phrasal heads as identified by the AM algebra. This occurs in constructions such as coordination and copula, what we term \textit{linker} problems, in which one MR ignores the central \textit{linker} (coordinator or copula verb), directly connecting the two linked elements, while another marks it as the central element, or root of the subgraph or head of the dependency subtree. A potential solution for such variation is to introduce multi-source root as-graphs into the algebra; this, however, would result in the algebra not predicting a unique AM dependency tree from the constants alone. \ld{Others look over this description and add, please! I'm getting confused with multiple-root graphs and double duty root/source nodes.} \ak{You have to expect that the reader has never seen the AM algebra before. Complications like this cannot be explained without showing an example and talking it through in detail. As a general rule, it is better to either explain a technical point completely or not at all. Explaining it halfway almost never works.}

%\jg{Another thing I realized is that by allowing the root source to be at the same node as another source, we don't always get a unique AM dep tree anymore just from the constants. That's not necessarily a bad thing since we can probably just choose the AM dep tree that looks most like the ones from the other corpora (so in a sense it's a good thing), but we'll have to figure out how to do this on a technical level.}

%Describe challenges in updating the AM algebra: double-duty root/source nodes, multiple-root graph question, discrepancies where one graphbank ignores an element \ml{Matthias} and \jg{Jonas}. 

Though these general patterns are present in our intermediate AM dependency trees and corresponding supertags, we still find subtle differences in how these patterns are actualized in the original graph structures. \ld{Pia can perhaps spell out the observation commented out above here.} We are also unable to account for all constructions that adhere to these patterns, given the manual nature of our methodology; future work will address the challenge of automating this process.  Here, we discuss four key linguistic phenomena that exhibit overlapping structural patterns to illustrate how we then unify them: negation (section \ref{subsec:negation}), copula (section \ref{subsec:copula}), coordination (section \ref{subsec:coordination}), and prepositions (section \ref{subsec:prepositions}). As presented here, these phenomena are specific to English, and we thus define the linguistic criteria for each in the relevant section. We discuss how these criteria and unification methods relate to cross-linguistic representations in section \ref{sec:discussion}.






%\ld{Use nice tables that Pia had in her presentation on Jan. 22} \pw{these tables are specific to our AM dependency trees, not the graph itself. However, we could probably extend it to the graphs in some cases}
\pw{do we need an extra paragraph/section about interactions of these phenomena?}



\subsubsection{Negation}\label{subsec:negation} 

\ak{Above you linked the linguistic considerations with the patterns. Here you say ``we address negation \ldots''. Perhaps we can make the two ways of motivating the constructions we care about more coherent. / Why is it okay to limit ourselves to a specific type of negation? Can we link this to frequency?}
We address negation constructions in which we can identify the negator as a separate lexical item. This includes negation of phrasal heads (primarily main and auxiliary verbs) with \textit{not} (see below); and adverbial negation with \textit{never}. Noun phrase negation with \textit{no} is treated in the same manner as determiners. We do not consider negation in MWEs or double negation constructions. Negation commonly interacts with other constructions such as auxiliary verbs and copula, often in complex manners, which we discuss in section \ref{subsec:interaction}.

The main design choice for negation in a MR is if it acts as head or as modifier of what it negates.
All SDP frameworks treat NP-internal negation as modification (\textit{not all of those parcels}, \textit{no planner}). For negation of main and auxiliary verbs, we find that PSD and PAS treat the negation as modifier as well, while DM usually considers the negation to be the head (see figure \ref{fig:negationDesignChoices}). However, there are exceptions, most notably relative clauses, in which DM also treats the negation as a modifier of the verb (\textit{the boy who did not survive}).

As unifying solution, we choose to make the negation the head. This requires changes of the AM dependency trees denoting PAS and PSD graphs, and DM graphs with relative clauses. The transformation involves reversing the edge between the negation and negated word and applying instead of modifying. In terms of as-graph for the negation, this means that we place the root-source on the node that already has the neg-source. Consequently, the negated word still contributes the root to the resulting graph. The transformation process is illustrated in figures \ref{fig:negationOld} and \ref{fig:negationUniform}. To preserve well-typedness, we ensure that the requirement at the neg-source matches the type the negated subtree evaluates to; in figure \ref{fig:negationUniform} the subtree rooted in \textit{sleep} evaluates to the empty type, which matches the requirement at the neg-source of the constant for \textit{not}.

\ml{TODO: mention similarity to type-raising? Mention that we used mod as source name before, now it's neg.}
\begin{figure}
    \centering
     \begin{subfigure}{0.32\textwidth}
    	\includegraphics[width=0.9\textwidth]{pics/negation/MaryNotSleep.pdf}
    	\caption{PSD (above) and DM (below)}
    	\label{fig:negationDesignChoices}
    \end{subfigure}%
     \begin{subfigure}{0.32\textwidth}
		\includegraphics[width=0.9\textwidth]{pics/negation/old/sentence.pdf}
		\caption{AM dependency tree for PSD}
		\label{fig:negationOld}
	\end{subfigure}%
     \begin{subfigure}{0.32\textwidth}
		\includegraphics[width=0.9\textwidth]{pics/negation/new/sentence.pdf}
		\caption{Unified AM dependency tree for PSD}
		\label{fig:negationUniform}
	\end{subfigure}
    \caption{Handling of negation. The two AM dependency trees evaluate both to the PSD graph.}
    \label{fig:negation}
\end{figure}


\begin{itemize}
    \item \ld{walk through example from Alexander's DMR talk} \pw{negation there is actually a combination of negation of the verb plus a modal verb (and verb subcategorizing for an embedded clause)} \ml{Isn't the example from the DMR talk a bit complicated for exposition here?}
    \item we observe two different design choices for representing negation of the verb:
    either the negation is the head of the verb (DM, other?) or negation is considered to be a modifier of the verb (PSD,PAS, DM in relative clauses, AMR, other?). However this is only a superficial difference if the AM algebra allows and additional source at the root node (example here)
    \item mention about discourse connectors: show similar pattern (in DM head of main verb, in PSD modifier), but less clear and probably less frequent. More than one connector at a time (maybe compare to double negation?)  
\end{itemize}

\subsubsection{Copula}\label{subsec:copula}  
% for visuals maybe refer to AM heuristics -> Towards new heuristics -> partial summary -> slides 23-24

As described above, certain copula constructions are instances of the linker problem. The central linking element in a copula construction is the copula verb (here: \textit{to be}). This verb signals a relation between subject and predicate. The question of whether this signaling or linking function is worth to be represented in the MR is answered differently by the different MRs.

% Graphs
Whereas all three SDP MRs treat the copula verb as a transitive verb in case of a nominal predicate \pw{todo: verify? example?}(e.g. \textit{Cats are mammals}), the treatment of copula with an adjectival predicate (e.g. \textit{Cats are lazy}) differs: 
DM treats this construction equivalent to adnominal adjectives (\textit{Lazy cats}), therefore the `meaning' of the verb is not really visible in the graph under the assumption that the ARG1 edges pertains to the adjective. PSD and PAS, however, still encode the copula verb as a transitive verb thus differing from the structure of adnominal adjectives. PAS even exhibits an control-like structure, or, in other words, merges the DM and PSD treatment in one graph (cf.~fig.~\ref{fig:copulagraphs}).

\begin{figure}
	\centering
	\begin{subfigure}{.3\textwidth}
		\centering
		\includegraphics{pics/copula/copulaDMgraph}
		\caption{DM}\label{fig:copulaDMgraph}
	\end{subfigure}
	\begin{subfigure}{.3\textwidth}
		\centering
		\includegraphics{pics/copula/copulaPASgraph}
		\caption{PAS}\label{fig:copulaPASgraph}
	\end{subfigure}
	\begin{subfigure}{.3\textwidth}
		\centering
		\includegraphics{pics/copula/copulaPSDgraph}
		\caption{PSD}\label{fig:copulaPSDgraph}
	\end{subfigure}
	\caption{SDP graphs for the adjective copula illustrated for example sentence \textit{Cats are lazy}}\label{fig:copulagraphs}
\end{figure}

% Dependency trees (old ones)
From the AM dependency tree perspective, the copula verb is ignored in DM (adjectival case) and the subject and predicate are directly connected (fig.~\ref{fig:copulaDMdecomp}). PSD and PAS both treat the verb as the root with outgoing \app{s} and \app{o} edges to the subject and the predicate respectively (fig.~\ref{fig:copulaPASdecomp},\ref{fig:copulaPSDdecomp}).

\begin{figure}
	\centering
	\begin{subfigure}{.25\textwidth}
		\centering
		\includegraphics[scale=.7]{pics/copula/copulaPSDdecomp}
		\caption{PSD}\label{fig:copulaPSDdecomp}
	\end{subfigure}
	\begin{subfigure}{.3\textwidth}
		\centering
		\includegraphics[scale=.7]{pics/copula/copulaPASdecomp}
		\caption{PAS}\label{fig:copulaPASdecomp}
	\end{subfigure}
	\begin{subfigure}{.2\textwidth}
		\centering
		\includegraphics[scale=.7]{pics/copula/copulaDMdecompOld}
		\caption{DM -- old}\label{fig:copulaDMdecomp}
	\end{subfigure}
	\begin{subfigure}{.2\textwidth}
		\centering
		\includegraphics[scale=.7]{pics/copula/copulaDMdecompNew}
		\caption{DM -- new}\label{fig:copulaDMdecompNew}
	\end{subfigure}
	\caption{Decompositions for \textit{Cats are lazy}}\label{fig:copuladecomp}
\end{figure}

% correspondence to structural pattern?
The phenomenon described above is similar to the structural pattern code 031.
Its most frequent PoS tags (verbal) and lemma (\textit{be}) also points in this direction. To reiterate, the pattern 031 reflects the fact that DM ignores the copula verb node (code 0), but PAS exhibits a control-like triangle structure (code 3) and finally, PSD uses a transitive verb structure (code 2).\pw{skip this paragraph or could we be more precise?}

% (Possible) Changes: (new dependency tree)
We unify the AM dependency trees by adding a supertag for the copula verb in DM: This supertag consists of one root node with an o source, requiring an s-source (see fig.~\ref{fig:copulaDMdecompNew}). This solution allows us to use the same DM adjective supertag for adnominal and predicative uses.
\pw{do we want to discuss other possible solutions? (see comments below)}
%If we would like to unify the AM dependency trees we have to decide on the goal dependency tree. We present three possible solutions:\pw{elaborate on solutions, maybe add figure}
%\begin{enumerate}
%    \item Solution one reanalyses DM and requires an additional source at the root node (one node blob), goal dependency tree is that of PSD and PAS.
%    \item Solution two would closely mirror the coordination solution \pw{check at end: still true}: we stick with the PSD and PAS dependency tree and reanalyse DM such that the copula verb receives a blob with a form standalone edge with at least one source at each attached node.
%    \item Solution three favors the DM dependency tree and reanalyses PAS and PSD. \pw{maybe difficult or impossible if we want to modify the adjective? but AM algebra doesn't need to be changed to allow additional source at root?}
%\end{enumerate}
%We choose solution 1 \pw{to do: explain why} (fig.~\ref{fig:copulaDMdecompNew}).

% Outlook: more MRs: AMR and EDS?
\ld{maybe add a sentence about EDS and AMR?}
We suspect that EDS would pattern with DM. AMR seems to exhibit the DM adjectival style for both adjectives and nouns in predicate position. But this needs further investigation.
% PW: just compared 'The sky is blue' and 'The sky is the limit' using the web demo of amparser

\pw{further specify phenomenon: what about participle vs adjective, PPs in predicate position, comparatives, existential constructions (\textit{There is})?}

\subsubsection{Coordination}\label{subsec:coordination} 

We consider coordinate phrases to be structures that link two or more elements of similar nature (NPs, VPs, APs, clauses), typically with a coordinating conjunct such as \textit{and}, \textit{but}, or \textit{or}. Coordinate phrases can occupy various syntactic positions (e.g. subject, object, modifier), possess distinct semantic interpretations (e.g. joint, split), and introduce scope ambiguities depending on the makeup of the conjuncts, all of which raises the question of if and how to treat them uniformly. %\cite[p.~919]{oepen-etal-2015-semeval}
\newcite{oepen-etal-2015-semeval} describe how the three SDP graphbanks distinctly encode coordination: DM uses a chain structure to connect the conjuncts via special conjunction edges (e.g. \textit{\_and\_c} or \textit{conj}); PSD identifies the last conjunction as the head with outgoing edges to all conjuncts; and PAS uses a binary branching structure. \pw{do we need a visual here for 3way conjunction?} This variation in graph structure is indicative of the theoretical complexity of coordinate structures, which also depends on the number of conjuncts in question \ld{cite}. Coordinate structures are nevertheless quite frequent in our data (27k instances; see table \ref{tab:patternfreq}). Here we present an initial analysis for unifying coordinate structures of two conjuncts across the graphbanks which make up approximately \pw{check number} 86 percent of all coordinations; we touch on possible solutions for the more challenging case of three or more conjuncts at the end of our discussion.\pw{do we?}


PSD and PAS both encode the meaning of coordination using a node (corresponding to the conjunction token) plus outgoing edges to its conjuncts (cf. fig.~\ref{fig:catMouse}). \pw{mention psd preprocessed}
Consequently, both MRs receive the same AM dependency tree and very similar supertags \pw{see Fig X} (see fig.~\ref{fig:coordDecompPAS} for PAS).
DM, however, chose to represent the coordination meaning only as an edge between the conjuncts (\textit{\_and\_c} edge in fig.~\ref{fig:catMouse}). The first conjunct is the head and `stands in' for the coordination as a whole. The AM dependency tree for DM differs from the other two MRs and we choose to change the DM decomposition in order to unify the compositional structure.
We do so by adding a supertag for the conjunction token (e.g. \textit{and}) containing the dedicated conjunction edge that was previously part of one of the conjuncts supertags (compare fig.~\ref{fig:coordDecompDMold} and \ref{fig:coordDecompDMnew}). The incident nodes use sources \textit{op1} and \textit{op2} to indicate the open positions for the conjuncts.\pw{note that again we need additional source at the root node?}
\begin{figure}
	\centering
	\begin{subfigure}{.32\textwidth}
		\centering
		\includegraphics[scale=.6]{pics/coordination/coordination_catmouseDMdecompOld}
		\caption{DM -- old decomposition}\label{fig:coordDecompDMold}
	\end{subfigure}
	\begin{subfigure}{.32\textwidth}
		\centering
		\includegraphics[scale=.6]{pics/coordination/coordination_catmouseDMdecompNew}
		\caption{DM -- new decomposition}\label{fig:coordDecompDMnew}
	\end{subfigure}
	\begin{subfigure}{.32\textwidth}
		\centering
		\includegraphics[scale=.6]{pics/coordination/coordination_catmousePASdecomp}
		\caption{PAS -- decomposition}\label{fig:coordDecompPAS}
	\end{subfigure}
	\caption{DM and PAS AM dependency trees for \textit{The cat and the mouse}}\label{fig:coordDecomp}
\end{figure}



The chosen representation also impacts how ambiguities are treated: While the structure used by PAS and PSD easily allows to distinguish between adjuncts with scope above and below the coordination (see fig.~\ref{fig:greentreesPAS} for PAS), the DM representation is underspecified with respect to certain scope ambiguities (see fig.~\ref{fig:greentreesDM}): an edge modifying the first, `head', conjunct can either modify the meaning of only the first conjunct or the coordination phrase as a whole. The scope ambiguity is also reflected in the AM dependency tree: the \modify{mod} edge could either connect the adjective with the conjunction (wide scope) or with one of the two conjuncts (narrow scope). As a consequence our changes allow two AM dependency trees for this phrase, both evaluating to the same DM graph, but to different PAS and PSD graphs. \pw{todo: show AM dependency trees?}
\pw{move this to the discussion section?}
\begin{figure}
	\centering
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics{pics/coordination/coordination_greentreesDMgraph}
		\caption{DM: same graph for narrow and wide scope}\label{fig:greentreesDM}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics{pics/coordination/coordination_greentreesPASgraphs}
		\caption{PAS: narrow (above) and wide (below) scope graphs}\label{fig:greentreesPAS}
	\end{subfigure}
	\caption{DM and PAS graphs for the coordination phrase \textit{Green trees and bushes}}\label{fig:greentrees}
\end{figure}

\pw{do we need more technical details of how we detect binary coordination?}
\pw{mention instance of linker problem? mention correspondence to structural pattern 011?}. 
\pw{mention multiple conjuncts here or in discussion? what about other MRs like AMR?}
%\begin{itemize}
%    \item Are there differences? among coordination of different types (VP, NP, AP) and in different positions (subject, object, modifier)? \todo{not answered yet}
%    \item Are there differences? Joint (\textit{My friend and colleague \textbf{is}...}) vs. split \textit{My friend and colleague \textbf{are}...}) readings. Do MRs distinguish these? \todo{not answered yet}
%    \item \pw{question} do we need more technical details about how we identify binary coordination? (using CC pos tag in DM, counting outgoing app op edges in psd, and whether there is a coord dependency edge in DM between the two conjuncts according to PSD
%    \item More than two conjuncts: Frequency and problems
%    \item Ambiguities of various kinds: 
%    (1) Multiple coordination (ambiguities here?) E.g. \textit{Charlie is tall, smart, and loves chocolate.} 
%    (2) adjuncts and readings E.g.~\textit{The green trees and bushes} in graph underspecified or one reading only? 
%    (3) \ld{to do: coordination and ambiguities}
%\end{itemize}


\subsubsection{Prepositions}\label{subsec:prepositions}

Though typically understood as a single morphosyntactic class in English, prepositions are notoriously polysemous \cite{schneider-18}. For our purposes, we analyze prepositions by distinct classes based on their POS tags and the constructions in which we find them: (i) possessives (typically \textit{of}); (ii) \textit{to}-infinitives; (iii) verb particles; and (iv) ``true'' prepositions, which include all other PPs. Prepositions often occur in MWEs, which we address if they fall into a structural pattern of the classes above. \ld{examples?}
